Greed is All You Need: An Evaluation of Tokenizer Inference Methods

While subword tokenizers such as BPE and WordPiece are typically used to build vocabularies for NLP models, the method of decoding text into a sequence of tokens from these vocabularies is often left unspecified, or ill-suited to the method in which they were constructed. We provide a controlled analysis of seven tokenizer inference methods across four different algorithms and three vocabulary sizes, performed on a novel intrinsic evaluation suite we curated for English, combining measures rooted in morphology, cognition, and information theory. We show that for the most commonly used tokenizers, greedy inference performs surprisingly well; and that SaGe, a recently-introduced contextually-informed tokenizer, outperforms all others on morphological alignment.

==> 99_latex_tips.tex <==

\uvp{\small
Some of my \LaTeX{} rules:
Full parenthetical citations (\texttt{\textbackslash{}cite} or \texttt{\textbackslash{}citep}) are preceded by a NBSP (tilde).
Each sentence gets its own source line (so it can be easily found, moved around, commented out).
We use \say{\texttt{\textbackslash{}say}} for quotes.
We don't use \texttt{\textbackslash{}subsubsections}---stuff below \texttt{\textbackslash{}subsection} gets \texttt{\textbackslash{}paragraph}.
We don't use \texttt{\textbackslash{}vspace} and its friends, definitely not in drafts.
When we have enough prose in a section (or sooner, whatever's convenient), we extract it to its own file.
\url{http://detexify.kirelabs.org/classify.html} is a life-saver.
We use macros for names and terms that might change,https://www.overleaf.com/project/6582b013e631fd8cfc095a29 like system names, and for inconveniently long but often-used phrases.
Numbers in the body of the text don't get put in mathmode.
Tables: no vertical lines, ever.
Minimal horizontal lines, using the \texttt{\textbackslash{}booktabs} extension (toprule and bottomrule in borders, midrule below legend and between coarse-grain row groups).
Anything that was published in a peer-reviewed venue is cited by its published venue, not arXiv.
If it was in an ACL-indexed venue, all you have to do is look it up on the anthology website (I have a Chrome shortcut for anthology search) and single-click-copy the bibkey, since we have the bib file already. Example:~\cite{klymenko-etal-2022-differential}.
For more: \href{https://medium.com/@vered1986/tips-for-writing-nlp-papers-9c729a2f9e1f}{here.}}

